Bravais colourings of planar modules with N-fold symmetry

The first step in investigating colour symmetries for periodic and aperiodic systems is the determination of all colouring schemes that are compatible with the symmetry group of the underlying structure, or with a subgroup of it. For an important class of colourings of planar structures, this mainly combinatorial question can be addressed with methods of algebraic number theory. We present the corresponding results for all planar modules with N-fold symmetry that emerge as the rings of integers in cyclotomic fields with class number one. The counting functions are multiplicative and can be encapsulated in Dirichlet series generating functions, which turn out to be the Dedekind zeta functions of the corresponding cyclotomic fields.

==> elements.tex <==
%Zeitschrift fuer Kristallographie, Oldenbourg Muenchen

\renewcommand{\Title}{Bravais colourings of planar modules with 
$\boldsymbol{N}$-fold symmetry}        

\renewcommand{\AuthorsComplete}{Michael Baake$^{\mathrm{I},*}$ and 
Uwe Grimm$^{\mathrm{II}}$}   

\renewcommand{\CorrespondenceAuthor}{(e-mail: mbaake@math.uni-bielefeld.de)} 
                   % absolutely preferred: (email) only

\renewcommand{\InstitutionOne}{Fakult\"{a}t f\"{u}r Mathematik, 
Universit\"{a}t Bielefeld, Postfach 100131, 33501 Bielefeld, 
Germany}    

\renewcommand{\InstitutionTwo}{Department of Mathematics, 
The Open University, Walton Hall, Milton Keynes MK7 6AA, UK}     

\renewcommand{\SayThanks}{}

\renewcommand{\Abstract}{The first step in investigating 
colour symmetries for periodic and aperiodic systems is the
determination of all colouring schemes that are compatible with the
symmetry group of the underlying structure, or with a subgroup of
it. For an important class of colourings of planar structures, this
mainly combinatorial question can be addressed with methods of
algebraic number theory. We present the corresponding results for all
planar modules with $N$-fold symmetry that emerge as the rings of
integers in cyclotomic fields with class number one. The 
counting functions are multiplicative and can be encapsulated in
Dirichlet series generating functions, which turn out to be the
Dedekind zeta functions of the corresponding cyclotomic fields.}


%%%%%%%%%%%%%%%%%%%%%%% for publisher only %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Paperreceived}{2003}
\renewcommand{\Paperaccepted}{2003}
\setcounter{Papervolume}{0}

\renewcommand{\Authors}{M. Baake and U. Grimm}

\renewcommand{\cleanTitle}{Bravais colourings of planar modules with 
$N$-fold symmetry}
\renewcommand{\shortAuthors}{Baake and Grimm}
\renewcommand{\shortTitle}{Bravais colourings of planar modules}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\endinput








